Improved Rates for Derivative Free Gradient Play in Strongly Monotone Games

The influential work of Bravo et al. 2018 shows that derivative free play in strongly monotone games has complexity $O(d^2/\varepsilon^3)$, where $\varepsilon$ is the target accuracy on the expected squared distance to the solution. This note shows that the efficiency estimate is actually $O(d^2/\varepsilon^2)$, which reduces to the known efficiency guarantee for the method in unconstrained optimization. The argument we present simple interprets the method as stochastic gradient play on a slightly perturbed strongly monotone game.

==> makefile <==
# set latexfile to the name of the main file without the .tex
latexfile = 2022arxiv
# put the names of figure files here.  include the .eps
#figures =
# if no references, run "touch latexfile.bbl; touch referencefile.bib"
# or delete dependency in .dvi and tarball sections
referencefile = 2022coltrefs

TEX = pdflatex

# support subdirectories
VPATH = Figs

# reruns latex if needed.  to get rid of this capability, delete the
# three lines after the rule.  Delete .bbl dependency if not using
# BibTeX references.
# idea from http://ctan.unsw.edu.au/help/uk-tex-faq/Makefile
$(latexfile).pdf : $(figures) $(latexfile).tex
#$(latexfile).dvi : $(figures) $(latexfile).tex $(latexfile).bbl
	while ($(TEX) $(latexfile) -synctex=1 ; \
	grep -q "Rerun to get cross" $(latexfile).log ) do true ; \
	done


# keep .eps files in the same directory as the .fig files
#%.eps : %.fig
#	fig2dev -L eps $< > $(dir $< )$@

#$(latexfile).pdf : $(latexfile).ps
#	ps2pdf $(latexfile).ps $(latexfile).pdf

#pdf : $(latexfile).pdf

#$(latexfile).ps : $(latexfile).dvi
#	dvips $(latexfile)

#ps : $(latexfile).ps

# make can't know all the sourcefiles.  some file may not have
# sourcefiles, e.g. eps's taken from other documents.
#$(latexfile).tar.gz : $(figures) $(latexfile).tex $(referencefile).bib
#	tar -czvf $(latexfile).tar.gz $^

#tarball: $(latexfile).tar.gz



clean:
	#rm $(latexfile).aux $(latexfile).log $(latexfile).pdf
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk

fixpdf:
	gs -dSAFER -dBATCH -dNOPAUSE  -sDEVICE=pdfwrite -sOutputFile=fixed.pdf $(latexfile).pdf

mpdf:
	$(TEX) $(latexfile).tex; skim $(latexfile).pdf

mbib:
	$(TEX) $(latexfile).tex; bibtex $(latexfile); $(TEX) $(latexfile).tex; $(TEX) $(latexfile).tex; skim $(latexfile).pdf

cleanit:
	#rm $(latexfile).aux $(latexfile).log $(latexfile).pdf
	rm -f *.swp

cpall:
	make mpdf; skim $(latexfile).pdf

